Deep Learning for Cross-Domain Data Fusion in Urban Computing: Taxonomy, Advances, and Outlook

As cities continue to burgeon, Urban Computing emerges as a pivotal discipline for sustainable development by harnessing the power of cross-domain data fusion from diverse sources (e.g., geographical, traffic, social media, and environmental data) and modalities (e.g., spatio-temporal, visual, and textual modalities). Recently, we are witnessing a rising trend that utilizes various deep-learning methods to facilitate cross-domain data fusion in smart cities. To this end, we propose the first survey that systematically reviews the latest advancements in deep learning-based data fusion methods tailored for urban computing. Specifically, we first delve into data perspective to comprehend the role of each modality and data source. Secondly, we classify the methodology into four primary categories: feature-based, alignment-based, contrast-based, and generation-based fusion methods. Thirdly, we further categorize multi-modal urban applications into seven types: urban planning, transportation, economy, public safety, society, environment, and energy. Compared with previous surveys, we focus more on the synergy of deep learning methods with urban computing applications. Furthermore, we shed light on the interplay between Large Language Models (LLMs) and urban computing, postulating future research directions that could revolutionize the field. We firmly believe that the taxonomy, progress, and prospects delineated in our survey stand poised to significantly enrich the research community. The summary of the comprehensive and up-to-date paper list can be found at https://github.com/yoshall/Awesome-Multimodal-Urban-Computing.

==> Tables/dataset_table_backup_hxx.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
%\usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \usepackage[normalem]{ulem}
% \useunder\url{ine}\url{}{}
\begin{table*}[htbp]
\resizebox{\textwidth}{!}{%
%\toprule[1pt]
\begin{tabular}{c|c|c|cll}
\toprule[2.0pt]
\specialrule{0.1em}{0.3em}{0.2em} %
%\midrule
 &
   &
   &
   &
   \\
\multirow{-2}{*}{\textbf{Category}} &
  \multirow{-2}{*}{\textbf{Content}} &
  \multirow{-2}{*}{\textbf{Format}} &

  \multirow{-2}{*}{\textbf{Dataset}} &
  \multirow{-2}{*}{\textbf{Link}} &
  \multirow{-2}{*}{\textbf{Reference}} \\ \midrule[1.5pt]
 & 
&
   &
  ArcGIS &
  {\color[HTML]{330001} \url{ https://developers.arcgis.com}} &
  \cite{liu2023knowledge} \\
 & &
   &
  PlanetScope (satellite images) &
  {\color[HTML]{330001} \url{ https://developers.planet.com/docs/data/planetscope/}} &
  \cite{li2022predicting} \\
 & &
   &
  Google Earth (satellite images) &
  {\color[HTML]{330001} \url{ https://developers.google.com/maps/documentation/}} &
  \begin{tabular}[c]{@{}l@{}}\cite{jenkinsUnsupervisedRepresentationLearning2019}\end{tabular} \\
 & &
   &
  OpenStreetMap (satellite images) &
  {\color[HTML]{330001} \url{ https://www.openstreetmap.org/}} &
  \cite{yin2023multimodal} \\
 &
  \multirow{-5}{*}{Satellite Image} &
  \multirow{-5}{*}{Image} &
  Baidu Maps( satellite images) &
  {\color[HTML]{330001} \url{ https://lbsyun.baidu.com}} &
  \begin{tabular}[c]{@{}l@{}}\cite{yangDuAREAutomaticRoad2022,xiaoContextualMasterslaveFramework2023}\end{tabular} \\ \cmidrule{2-6} 
 & &
   &
  Baidu Map API (street view images) &
  {\color[HTML]{330001} \url{ https://lbsyun.baidu.com}} &
  \begin{tabular}[c]{@{}l@{}}\cite{liu2023knowledge,jiangITVInferringTraffic2021}\end{tabular} \\
 & &
   &
  Google Street API (street view images) &
  {\color[HTML]{330001} \url{ https://developers.google.com/maps/}} &
  \begin{tabular}[c]{@{}l@{}}\cite{liu2023knowledge,afyouni2022multi}\end{tabular} \\
 &
  \multirow{-3}{*}{Street View Image} &
  \multirow{-3}{*}{Image}&

  Tencent (street view images) &
  {\color[HTML]{330001} \url{ https://lbs.qq.com/tool/streetview/index.html}} &
  \cite{huang2023comprehensive}\\ \cmidrule{2-6} 
 & &
   &
  Tencent Map Service(POIs) &
  {\color[HTML]{330001} \url{ https://lbs.qq.com/getPoint/}} &
  \begin{tabular}[c]{@{}l@{}}\cite{xiFirstLawGeography2022b,ruan2022service}\end{tabular} \\
& &
   &
  WeChat POIs &
  {\color[HTML]{330001} \url{ https://open.weixin.qq.com}} &
 \cite{wangSpatiotemporalUrbanKnowledge2021} \\
& &
   &
  Baidu Map POIs) &
  {\color[HTML]{330001} \url{ https://lbsyun.baidu.com}} &
  \begin{tabular}[c]{@{}l@{}}\cite{liPredictingMultilevelSocioeconomic2022a,liuCharacterizingForecastingUrban2023,liuJointRepresentationLearning2019,huangERNIEGeoLGeographyandlanguagePretrained2022,xiaoContextualMasterslaveFramework2023}\end{tabular} \\
& &
   &
  NYC Open Data (POIs) &
  {\color[HTML]{330001} \url{ https://opendata.cityofnewyork.us/}} &
  \begin{tabular}[c]{@{}l@{}}\cite{lin2019deepstn+,wang2021gsnet,bingPretrainedSemanticEmbeddings2023,zhangRegionEmbeddingIntra2023,wangTrafficAccidentRisk2023}\end{tabular} \\
& &
   &
  Foursquare &
  {\color[HTML]{330001} \url{ https://developer.foursquare.com/docs/checkins/checkins}} &
  \begin{tabular}[c]{@{}l@{}}\cite{bingPretrainedSemanticEmbeddings2023,zhaoAnnotatingPointsInterest2016a,balsebreGeospatialEntityResolution2022,chenInformationCoverageLocation2015a,huangExploitingSpatialtemporalsocialConstraints2016b,jenkinsUnsupervisedRepresentationLearning2019}\end{tabular} \\
& &
   &
  Wikipedia POIs &
  {\color[HTML]{330001} \url{ https://www.wikipedia.org}} &
  \cite{zhaoPhoto2TripExploitingVisual2021} \\
& &
   &
  AMap Service (POIs) &
  {\color[HTML]{330001} \url{ https://lbs.amap.com}} &
  \cite{baiGeographicMappingUnsupervised2023a} \\
& &
   &
  Yelp POIs &
  {\color[HTML]{330001} \url{ https://www.yelp.com/developers}} &
  \begin{tabular}[c]{@{}l@{}}\cite{balsebreGeospatialEntityResolution2022,zhaoPGeoTopicDistributedSolution2020,zhao2016towards}\end{tabular} \\
& &
   &
  {Dianping.com POIs} &
  {\color[HTML]{330001} \url{ https://api.dianping.com/}} &
  \begin{tabular}[c]{@{}l@{}}\cite{chandraNodeSense2VecSpatiotemporalContextaware2021,duGeofirstLawLearning2019}\end{tabular} \\
& &
   &
  Weibo POI &
  {\color[HTML]{330001} \url{ https://open.weibo.com/wiki/API}} &
  \begin{tabular}[c]{@{}l@{}}\cite{chandraNodeSense2VecSpatiotemporalContextaware2021,keerthichandraCollectiveEmbeddingFeature2020a,gaoDualgrainedHumanMobility2023b}\end{tabular} \\
& &
   &
  Flickr (POI) &
  {\color[HTML]{330001} \url{ https://www.flickr.com/services/developer/api/}} &
  \cite{heJointContextawareEmbedding2019}\\
& 
  \multirow{-13}{*}{POIs} &
   \multirow{-13}{*}{Point Vector} &
  Bing Map POIs &
  {\color[HTML]{330001} \url{ https://www.bingmapsportal.com}} &
  \begin{tabular}[c]{@{}l@{}}\cite{chenCrosscityFederatedTransfer2022}\end{tabular} \\ \cmidrule{2-6} 
 &&
   &
  US Census Bureau &
  {\color[HTML]{330001} \url{ https://www.census.gov/data.html}} &
  \cite{zhangRegionEmbeddingIntra2023} \\
\multirow{-23}{*}{\textbf{Geographical Data}} &
  \multirow{-2}{*}{Map} &
  TODD&
  { OpenStreetMap(digital maps)} &
  {\color[HTML]{330001} \url{ https://www.openstreetmap.org/}} &
  \begin{tabular}[c]{@{}l@{}}\cite{yinMultitaskLearningFramework2020a,balsebreGeospatialEntityResolution2022,luoLetTrajectoriesSpeak2021,yuanEffectiveJointPrediction2021,gengMultimodalGraphInteraction2019}\end{tabular} \\ \midrule
 &&
   &
  California-PEMS &
  {\color[HTML]{330001} \url{ http://pems.dot.ca.gov}} &
  \cite{}\\
 &&
   &
  METR-LA &
  {\color[HTML]{330001} \url{ https://www.metro.net}} &
  \cite{}\\
 &&
   &
  Large-ST &
  {\color[HTML]{330001} \url{ https://github.com/liuxu77/LargeST}} &
  \cite{}\\
 &&
   &
  Shenzhou UCar &
  {\color[HTML]{330001} \url{ https://bit.ly/2MG47xz}} &
  \cite{guoForcedirectedApproachSeeking2022}\\
 &&
   &
  DiDi (Traffic flows) &
  {\color[HTML]{330001} \url{ https://outreach.didichuxing.com/research/opendata/}} &
  \begin{tabular}[c]{@{}l@{}}\cite{yuanEffectiveJointPrediction2021,luoLetTrajectoriesSpeak2021,rajehModelingMultiregionalTemporal2023,yao2022trajgat,tedjopurnomo2021similar}\end{tabular} \\ 
 &&
   &
  Chicago Transportation&
  {\color[HTML]{330001} \url{ https://data.cityofchicago.org/}} &
  \begin{tabular}[c]{@{}l@{}}\cite{wang2021gsnet,wangTrafficAccidentRisk2023,jenkinsUnsupervisedRepresentationLearning2019}\end{tabular} \\
 &&
   &
  Taxi Trajectory Shenzhen &
  {\color[HTML]{330001} \url{ https://github.com/cbdog94/STL}} &
  \begin{tabular}[c]{@{}l@{}}\cite{huangComprehensiveUrbanSpace2023a,wuMiningSpatiotemporalReachable2017}\end{tabular} \\
 &&
   &
  NYC open data (Taxi trips) &
  {\color[HTML]{330001} \url{ https://opendata.cityofnewyork.us/how-to/}} &
  \begin{tabular}[c]{@{}l@{}}\cite{zhangMultiviewJointGraph2021a,zhangRegionEmbeddingIntra2023}\end{tabular} \\

 &&
   &
  Xiamen Taxi &
  {\color[HTML]{330001} \url{ https://data.mendeley.com/datasets/6xg39x9vgd/1}} &
  \begin{tabular}[c]{@{}l@{}}\cite{youPANDAPredictingRoad2022,chenUVLensUrbanVillage2021,jiangITVInferringTraffic2021,chenRADARRoadObstacle2018}\end{tabular} \\
 &&
   &
  TaxiBJ &
  {\color[HTML]{330001} \url{https://goo.su/aQyjTAz}} &
  \begin{tabular}[c]{@{}l@{}}\cite{liangFinegrainedUrbanFlow2021,bai2019stg2seq,qu2022forecasting,jiSelfsupervisedSpatiotemporalGraph2023,zhangMultiviewJointGraph2021a,fuEfficientRegionEmbedding2019}\end{tabular} \\ 

 &&
   &
  Grab-Posisi &
  {\color[HTML]{330001} \url{ https://goo.su/W3yD5m}} &
  \begin{tabular}[c]{@{}l@{}}\cite{yinMultimodalDeepLearning2023a,yinMultitaskLearningFramework2020a}\end{tabular} \\

 &
  \multirow{-10}{*}{ Traffic trajectory} &
  \multirow{-10}{*}{Trajectory} &
  BikeNYC &
  {\color[HTML]{330001} \url{ https://citibikenyc.com/}} &
  \begin{tabular}[c]{@{}l@{}}\cite{lin2019deepstn+,bai2019stg2seq,qu2022forecasting,jiSelfsupervisedSpatiotemporalGraph2023}\end{tabular} \\ \cmidrule{2-6} 
  
 &
  &
  &
  OpenStreetMap &
  {\color[HTML]{330001} \url{ https://www.openstreetmap.org}} &
  \cite{yuan2021effective} \\ 


   &
  &
 &
  OpenStreetMap &
  {\color[HTML]{330001} \url{ https://www.openstreetmap.org}} &
  \cite{yuan2021effective} \\ 
   &
  &
 &
  OpenStreetMap &
  {\color[HTML]{330001} \url{ https://www.openstreetmap.org}} &
  \cite{yuan2021effective} \\ 


   &
  &
  &
  OpenStreetMap &
  {\color[HTML]{330001} \url{ https://www.openstreetmap.org}} &
  \cite{yuan2021effective} \\ 

   &
  \multirow{-4}{*}{Taffic Flow}&
  \multirow{-4}{*}{TODO}&
  OpenStreetMap &
  {\color[HTML]{330001} \url{ https://www.openstreetmap.org}} &
  \cite{yuan2021effective} \\   \cmidrule{2-6}

  &
 Logistics&
  TODO&
  JD Logistics in Bejing &
  {\color[HTML]{330001} \url{ https://www.openstreetmap.org}} &
  \cite{yuan2021effective} \\ \cmidrule{2-6}


   &
  &
  &
  OpenStreetMap &
  {\color[HTML]{330001} \url{ https://www.openstreetmap.org}} &
  \cite{yuan2021effective} \\ 


  \multirow{-17}{*}{\textbf{Traffic Data}} &
  \multirow{-2}{*}{Road Network} &
  \multirow{-2}{*}{TODO}&
  OpenStreetMap &
  {\color[HTML]{330001} \url{ https://www.openstreetmap.org}} &
  \cite{yuan2021effective} \\ \midrule
   &&
     &
    \multirow{2}{*}{Twitter (check-in \& geo-tagged tweets)} &
  \multirow{2}{*}{{\color[HTML]{330001} \url{ https://developer.twitter.com/en/docs}} }&
    \begin{tabular}[c]{@{}l@{}}\cite{bingPretrainedSemanticEmbeddings2023,zhaoAnnotatingPointsInterest2016a,zhao2016towards,yuan2017pred,vu2016geosocialbound,wu2015semantic,shen2018forecasting}\end{tabular} \\
  &&
     &
      &
        &
    \begin{tabular}[c]{@{}l@{}}\cite{wang2017computing,wang2016estimating,wang2016enhancing,wang2015citywide,miyazawa2019integrating,liuSpatiotemporalActivityModeling2022}\end{tabular} \\
   &&
     &
    \multicolumn{1}{c}{Common Crawl web pages} &
    {\color[HTML]{330001} \url{ https://registry.opendata.aws/commoncrawl/}} &
    \cite{zhao2020pgeotopic} \\
   &&
     &
    \multicolumn{1}{c}{Yelp user reviews} &
    {\color[HTML]{330001} \url{ https://www.yelp.com/dataset}} &
    \begin{tabular}[c]{@{}l@{}}\cite{zhao2020pgeotopic,zhao2016towards}\end{tabular} \\
   &
    \multirow{-4}{*}{Text} &
    \multirow{-4}{*}{Text} &
    \multicolumn{1}{c}{Weibo Xiamen Traffic Police} &
    {\color[HTML]{330001} \url{http://open.weibo.com/developers/}} &
    \cite{you2022panda} \\ \cmidrule{2-6} 

   &&
     &
    \multicolumn{1}{c}{\multirow{-1}{*}{YFCC100M (geo-tagged photo)}} &
    \multirow{-1}{*}{{\color[HTML]{330001} \url{ https://goo.su/jzaDU}}} &
    \multirow{-1}{*}{\begin{tabular}[c]{@{}l@{}}\cite{zhao2017photo2trip,yin2021learning,heJointContextawareEmbedding2019}\end{tabular}} \\

   &&
     &
    \multicolumn{1}{c}{\multirow{-1}{*}{NUS-WIDE (geo-tagged photo)}} &
    \multirow{-1}{*}{{\color[HTML]{330001} \url{ https://goo.su/dWPQZcD}}} &
    \multirow{-1}{*}{\begin{tabular}[c]{@{}l@{}}\cite{yin2021learning,yin2019gps2vec}\end{tabular}} \\
   &
    \multirow{-3}{*}{Image\&Video} &
    \multirow{-3}{*}{Image\&Video} &
    \multicolumn{1}{c}{GeoUGV (geo-tagged mobile video)} &
    {\color[HTML]{330001} \url{ https://qualinet.github.io/databases/video/}} &
    \cite{lu2016geougv} \\ \cmidrule{2-6} 
   &&
     &
    \multicolumn{1}{c}{Jiepang user check-in} &
    {\color[HTML]{330001} \url{ https://jiepang.app/}} &
    \cite{fu2019efficient} \\
   &&
     &
    \multicolumn{1}{c}{Gowalla user location} &
    {\color[HTML]{330001} \url{ http://konect.cc/networks/loc-gowalla_edges/}} &
    \begin{tabular}[c]{@{}l@{}}\cite{chenInformationCoverageLocation2015a,yuan2017pred}\end{tabular} \\
  \multirow{-10}{*}{\textbf{Social Network Data}} &
    \multirow{-3}{*}{User’ Info.} &
        \multirow{-3}{*}{User’ Info.} &
    \multicolumn{1}{c}{WeChat BJ/SH user mobility} &
     {\color[HTML]{330001} \url{ https://open.weixin.qq.com/}} &
    \cite{wangSpatiotemporalUrbanKnowledge2021} \\ \midrule
&
  Crime&
  Time series&
  NYC Crime
  &{\color[HTML]{330001} \url{ https://opendata.cityofnewyork.us/}} &
  \cite{zhangMultiviewJointGraph2021a} \\ \cmidrule{2-6} 
&&
  &
  Land Use SG
  &{\color[HTML]{330001} \url{ https://www.ura.gov.sg/Corporate/Planning/Master-Plan}} &
  \cite{liUrbanRegionRepresentation2023} \\
&\multirow{-2}{*}{Land Use}
  &
  Time series
  &Land Use NYC
  &{\color[HTML]{330001} \url{ https://goo.su/puTuG}} &
  \cite{liUrbanRegionRepresentation2023} \\
  \cmidrule{2-6} 
\multirow{-4}{*}{\textbf{Demographic Data}} &
  Population &
  Time series &
  WorldPo&
  {\color[HTML]{330001} \url{ https://www.worldpop.org/}} &
  \begin{tabular}[c]{@{}l@{}}\cite{xiFirstLawGeography2022b,li2022predicting,baiGeographicMappingUnsupervised2023a}\end{tabular} \\ \midrule
 &&
   &
  TipDM China Weather Dataset &
  {\color[HTML]{330001} \url{ https://www.tipdm.org/}} &
  \cite{liu2022symbolic} \\
 &&
   &
  DarkSky weather &
  {\color[HTML]{330001} \url{ https://support.apple.com/en-us/102594}} &
  \cite{yuanEffectiveJointPrediction2021} \\
 &&
   &
  WeatherNY &
  {\color[HTML]{330001} \url{ https://opendata.cityofnewyork.us/}} &
  \cite{wang2021gsnet}\\
 &&
   &
  WeatherChicago &
  {\color[HTML]{330001} \url{ https://data.cityofchicago.org/}} &
  \cite{wang2021gsnet}\\
 &&
   &
  Weather Underground &
  {\color[HTML]{330001} \url{ https://www.wunderground.com/}} &
  \cite{youPANDAPredictingRoad2022}\\

 &&
   &
  DidiSY (weather, temperature, wind speed) &
  {\color[HTML]{330001} \url{ https://www.didiglobal.com/}} &
  \cite{bai2019spatio} \\
 &&
   &
  WD\_BJ (weather) &
  {\color[HTML]{330001} \url{ https://goo.su/DmHFHd}} &
  \cite{maHiSTGNNHierarchicalSpatiotemporal2022}\\
 &
 \multirow{-8}{*}{Meteorology}  &
 Time series&
  WD\_ISR \& WD\_USA (weather) &
  {\color[HTML]{330001} \url{ https://goo.su/RVhBA}} &
  \cite{maHiSTGNNHierarchicalSpatiotemporal2022}\\
  \cmidrule{2-6}
 &
  Greenery &
  Time series &
  Google Earth (tree coverage)&
  {\color[HTML]{330001} \url{ https://earth.google.com/}} &
  \cite{youPANDAPredictingRoad2022} \\
   \cmidrule{2-6}
\multirow{-10}{*}{\textbf{Environmental Data}} &
  Air Quality &
  Time series&
  UrbanAir &
{\color[HTML]{330001} \url{https://goo.su/hfzNB53}} &
  \cite{zheng2015Forecasting}\\ %\midrule
  \bottomrule[2.0pt]
\end{tabular}%

}
\caption{ Taxonomy and summary of open-sourced dataset used for multimodal urban computing}
\label{tab:dataset-table}
\end{table*}
